AdS_2/CFT_1 at finite density and holographic aspects of 2D black holes

In the present thesis, we study various models of 2D dilaton gravity known as JT gravity coupled with non-trivial gauge interactions (for instance $SU(2)$ Yang-Mills, quartic interactions between $U(1)$ gauge fields and Modmax interactions etc.). In particular, we investigate the effects of the non-trivial gauge couplings on the thermal properties of black holes and wormholes in two dimensions and compute various physical observables like entropy, free energy, etc. Further, we examine the possibilities of the Hawking-Page transition and wormhole to black hole phase transition in two dimensions. In addition, we also study the transformation properties of boundary stress-energy tensor under the diffeomorphism and $U(1)$ gauge transformation and hence compute the central charge associated with the 1D boundary theory.

==> empty.tex <==
\newpage
~\\
~\\

\thispagestyle{empty}
\cleardoublepage
\addtocounter{page}{-1}


==> empty1.tex <==
\newpage

~\\
~\\


\thispagestyle{empty}
\cleardoublepage
%\addtocounter{page}{-1}

